Run-Off Election: Improved Provable Defense against Data Poisoning Attacks

In data poisoning attacks, an adversary tries to change a model's prediction by adding, modifying, or removing samples in the training data. Recently, ensemble-based approaches for obtaining provable defenses against data poisoning have been proposed where predictions are done by taking a majority vote across multiple base models. In this work, we show that merely considering the majority vote in ensemble defenses is wasteful as it does not effectively utilize available information in the logits layers of the base models. Instead, we propose Run-Off Election (ROE), a novel aggregation method based on a two-round election across the base models: In the first round, models vote for their preferred class and then a second, Run-Off election is held between the top two classes in the first round. Based on this approach, we propose DPA+ROE and FA+ROE defense methods based on Deep Partition Aggregation (DPA) and Finite Aggregation (FA) approaches from prior work. We evaluate our methods on MNIST, CIFAR-10, and GTSRB and obtain improvements in certified accuracy by up to 3%-4%. Also, by applying ROE on a boosted version of DPA, we gain improvements around 12%-27% comparing to the current state-of-the-art, establishing a new state-of-the-art in (pointwise) certified robustness against data poisoning. In many cases, our approach outperforms the state-of-the-art, even when using 32 times less computational power.

==> figures/plots.tex <==
% !TEX root = ../main.tex
\begin{figure}[tbp]
  \centering
  \begin{subfigure}{1\linewidth}
    \centering
    \begin{minipage}{0.48\linewidth}
      \includegraphics[width=1\linewidth]{figures/certified_accuracy/cifar-k50.pdf}
    \end{minipage} 
    \begin{minipage}{0.48\linewidth}
      \includegraphics[width=1\linewidth]{figures/improvement/cifar-k50.pdf}
    \end{minipage}
    \caption{CIFAR-10 $(k=50)$}
    \label{fig:cifar10-k50}
  \end{subfigure}\\
  \begin{subfigure}{1\linewidth}
    \centering
    \begin{minipage}{0.48\linewidth}
      \includegraphics[width=1\linewidth]{figures/certified_accuracy/cifar-k250.pdf}
    \end{minipage} \hfill
    \begin{minipage}{0.48\linewidth}
      \includegraphics[width=1\linewidth]{figures/improvement/cifar-k250.pdf}
    \end{minipage} \hfill
    \caption{CIFAR-10 $(k=250)$}
    \label{fig:cifar10-k250}
  \end{subfigure}\\
  \begin{subfigure}{1\linewidth}
    \centering
    \begin{minipage}{0.48\linewidth}
      \includegraphics[width=1\linewidth]{figures/certified_accuracy/mnist-k1200.pdf}
    \end{minipage} \hfill
    \begin{minipage}{0.48\linewidth}
      \includegraphics[width=1\linewidth]{figures/improvement/mnist-k1200.pdf}
    \end{minipage} \hfill
    \caption{MNIST $(k=1200)$}
    \label{fig:mnist-k1200}
  \end{subfigure}\\
  \begin{subfigure}{1\linewidth}
    \centering
    \begin{minipage}{0.48\linewidth}
      \includegraphics[width=1\linewidth]{figures/certified_accuracy/gtsrb-k50.pdf}
    \end{minipage} \hfill
    \begin{minipage}{0.48\linewidth}
       \includegraphics[width=1\linewidth]{figures/improvement/gtsrb-k50.pdf}
    \end{minipage} \hfill
    \caption{GTSRB $(k=50)$}
    \label{fig:gtsrb-k50}
  \end{subfigure}\\
  \begin{subfigure}{1\linewidth}
    \centering
    \begin{minipage}{0.48\linewidth}
      \includegraphics[width=1\linewidth]{figures/certified_accuracy/gtsrb-k100.pdf}
    \end{minipage} \hfill
    \begin{minipage}{0.48\linewidth}
      \includegraphics[width=1\linewidth]{figures/improvement/gtsrb-k100.pdf}
    \end{minipage} \hfill
    \caption{GTSRB $(k=100)$}
    \label{fig:gtsrb-k100}
  \end{subfigure}\\
\caption{
The curves of certified fraction of different methods on different datasets.
\textbf{Left}: Certified fraction of \dparoe{}, \faroe{}, and FA with maximum value of $d$.
\textbf{Right}: The improvements of certified fraction from DPA to \dparoe{}, 
\faroe{}, and FA with the same $k$ and maximum $d$. 
}
\label{fig:certified_fraction}
\end{figure}



==> old-notes/old-main.tex <==
% !TEX root = ../main.tex
\subsection{Jan 20 trash}
\begin{algorithm}
  \caption{DPA algorithm \SF{not necessary; focus on ROE}}
  \label{alg:DPA}
  \begin{algorithmic}[1]
    \Require{Dataset $D \subseteq \mathcal{X} \times \mathcal{C}$, hash function $h : \mathcal{X} \to [k]$, test sample $x \in \mathcal{X}$.}
    \Ensure{Prediction of DPA for $x$.}
    \Function{\Train}{$D, h$}
      \For{$i\gets 1, \dots, k$}
        \State $D_i \gets \{x \in D: h(x) = i\}, \quad f_i \gets f_{D_i}$
      \EndFor
      \State \Return $\{f_i\}_{i=1}^{k}$
    \EndFunction
    \Function{\Predict}{$\{f_i\}_{i=1}^k, x$}
      \For{$c\in \mathcal{C}$}
        \State $N_c \gets \sum_{i=1}^k\ind{f_i(x) = c}$
      \EndFor
      \State \Return $\argmax_{c\in \mathcal{C}} N_{c}$
    \EndFunction
  \end{algorithmic}
\end{algorithm}

Given a test sample $x$,
DPA calculates the prediction vector
$\{f_i(x)\}_{i=1}^k$ 
and outputs the most frequent class as its final output.
Formally, letting
$N_c := \sum_{i=1}^k \ind{f_i(x)=c}$ denote
the number of models predicting $c$,
$DPA(D, x) = \argmax_{c\in \mathcal{C}} N_c$.
We assume that $\argmax$ breaks ties in lexicographic order,
i.e., it favors the class $c$ with the smaller index.
The pseudocode of DPA is written in Algorithm~\ref{alg:DPA}.
We note that $N_c$ implicitly depends on $D$, though we hide this dependence for convenience.

The partitioning of training set effectively creates
a sandbox against poisoning as the effect of each poisoned sample
is isolated in a single partition.
Since each poisoned sample can affect at most one base classifier,
the adversary can change at most $B$ votes.
As long as the prediction was chosen with a large enough \emph{margin} however,
this would not change the final prediction.

% \newcommand{\dpa}{\textnormal{DPA}}
\begin{theorem}\label{thm:dpa}
  \todo{Reword with rad.}
  Given a training set $D$ and an input $x$, 
  let $\cpred = \dpa(D, x)$, then for any training set $D'$, if
  \begin{align*}
    \dsym(D, D') < \ceil{\frac{\gap(\bN, \cpred, c)}{2}}
    ,
  \end{align*}
  holds for all $c\ne \cpred$, we have $DPA(D, x) = DPA(D', x)$.
\end{theorem}

While DPA produces a provable defense, we show that
it is wasteful in the way it utilizes the base classifiers.
For any single test sample $x$,
only the final prediction of each model is considered for prediction.
This effectively turns the prediction into a race between the top-two
classes and models not voting for these classes are ignored.
Indeed, when viewed as an \emph{election},
DPA corresponds to ``first-past-post'', which is widely known to be
especially problematic when the number of partitions is large,
as many models may not vote for the top two classes but
may still contain useful predictions about
which of the top two classes should be given as output.
This is reasonable because a binary classification task between the top two classes
is fundamentally an easier problem than multi-classification.
In the next section, we show how to better use the base classifiers
for obtaining a more robust prediction.

\subsection{Explanation, intuition}

By using the full logit-layer information for each model,
we are effectively increasing the number of base classifiers
involved in the final prediction,
which \emph{dilutes} the effect of each poisoned sample.
% \emph{without lowering their quality and without extra training cost.}
While this can also be done by either increasing $k$ or, as in
\cite{wang2022improved}, training with multiple hash functions,
this would either lower
the quality of the base models or
increase the training cost.
Our method does not suffer from either of these issues as we simply reuse the discarded classifiers.

A base assumption in our method is that the base classifiers
can reliably discern between the top two classes. 
This seems counterintuitive at first as these models
were not good enough to predict one of the top-two classes.
We note however that the classification task in the second round is
fundamentally easier and the models need to predict between
only two classes, whereas in round 1, they have to choose from $|\mathcal{C}|$ possible classes.
We, therefore, expect models to be useful in round 2, even if they were not
useful in round 1. This is validated by our results in Section \ref{sec:experiment},
where we see significant improvements over the current state of the art
with considerable computational gains.

\subsection{No more explain}
\begin{algorithm}[t]
  \caption{FA training \SF{push to appendix}}
  \label{alg:FA}
  \begin{algorithmic}[1]
    \Require{Dataset $D \subseteq \mathcal{X} \times \mathcal{C}$, hash functions $\hsplit : \mD \to [kd], \hspread: [kd] \to [kd]^d$.}
    \Ensure{Trained $\{f_i\}_{i=1}^{kd}$ classifiers.}
    \Function{\Train}{$D, \hsplit, \hspread$}
      \For{$i\gets 1, \dots, kd$}
        \State $D_{i} \gets \{x: i \in \hspread(\hsplit(x))\}, \quad f_i \gets f_{D_i}$
      \EndFor
      \State \Return $\{f_i\}_{i=1}^{kd}$
    \EndFunction
  \end{algorithmic}
\end{algorithm}


As discussed in \cite{wang2022improved}, by suitably choosing the hash function $\hspread$,
we can ensure that each dataset $D_i$ is comprised of $d$ distinct buckets. This means
that the size of each $D_i$ is roughly equal to $\frac{1}{k}|D|$. 
This means that we expect each base classifier to have the same accuracy as in DPA.
Since we are using $kd$ classifiers however, we expect the number of votes in 
each class, i.e., $\none_{c}$, to be scaled by a factor of $d$.
Crucially, however, the power of adversary \emph{does not} scale by a factor of $d$.
While each poison datapoint affects $d$ datasets, these $d$ datasets
are not controlled by the adversary. 
Indeed,
for the adversary's power to scale with $d$,
it needs to find buckets $b$ such that for all $f_i(x) = \cpred$ for all 
$i\in \hspread(b)$. These buckets are going to be limited however given the pseudorandom nature of $\hspread$.

\begin{algorithm}[t]
  \caption{ROE algorithm}
  \label{alg:ROE}
  \begin{algorithmic}[1]
    \Require{Trianed classifiers $\{f_i\}_{i=1}^k$, test sample $x \in \mathcal{X}$.}
    \Ensure{Prediction of Run-off election for $x$.}
    \Function{\Predict}{$\{f_i\}_{i=1}^k, x$}
      \State \textcolor{gray}{/* Round 1 */}
      \For{$c\in \mathcal{C}$}
        \State $\none_c \gets \sum_{i=1}^k\ind{f_i(x) = c}$
      \EndFor
      \State $c_1 \gets \argmax_{c} \none_c, \quad c_2 \gets \argmax_{c\ne c_1} \none_c$.
      \State \textcolor{gray}{/* Round 2 */}
      \State $\nrun_{c_1} \gets \sum_{i=1}^k \ind{f_i^{\logit}(x, c_1) > f_i^{\logit}(x, c_2)}$
      \State $\nrun_{c_2} \gets k - \nrun_{c_2}$
      \State \Return $\argmax_{c\in \{c_1, c_2\}} \nrun_{c}$
    \EndFunction
  \end{algorithmic}
\end{algorithm}

\section{Old main section}



Let $\cpred$ be the prediction of our method and
let $\csec$ be the other class that
was considered in round $2$, i.e.,
$\{\cpred, \csec\} = \{c_1, c_2\}$.
In order to change the prediction of our method,
the adversary needs to either eliminate the class $\cpred$ in the first round,
or ensure that it loses in the second round.
We therefore separately consider the two rounds and 
lower bound the number of poisoned samples the adversary needs
to eliminate $\cpred$. We then take the minimum of these two numbers as our final certificate.

\kpar{Round 1}
In order to eliminate $\cpred$ in the first round.
This means it needs to choose two classes $\{c'_1, c'_2\}$ such that
$\cpred \notin \{c'_1, c'_2\}$ and poison enough models such that
$\{c'_1, c'_2\}$ make it to Round 2 in the election. While in principle the adversary
can choose any pair from $\mC - \{\cpred\}$, we will show that it is sufficient
to consider $\{c'_1, c'_2\} = \{\csec, c_3\}$, where $c_3$ is
the \emph{third} class in the first round, i.e., $c_3 := \argmax_{c\notin \{c_1, c_2\}} \none_{c}$.
From now on, since we are considering two rounds,
we denote by $\bNfirst$ the vector that counts the number of votes in the first round, i.e., 
$\bN^{\rone} = (N^{\rone}_c)_{c\in \mC}$.

The minimum number of poisons necessary to ensure $\{\csec, c\}$ are chosen
in Round 1 can be calculated using a water-filling style argument.
The adversary first needs to change enough votes from $\cpred$ to $c$
to ensure $c_3$ beats $\cpred$, i.e., 
make the gap $\gap(\bNfirst, \cpred, c_3)$ non-positive.
Since each poisoned sample can change at most two votes, it needs to poison
at least $\cert^{\rone}_{c}$ points where 
\begin{align*}
  &\cert^{\rone}_1 := \ceil{\frac{\gap(\bNfirst, \cpred, c)}{2}}
  .
\end{align*}
If at this point $\csec$ also beats $\cpred$, then no more changes are necessary.
Otherwise, the adversary needs to keep changing votes from $\cpred$ to $\csec$ till this happens.
Obtaining a formal bound requires careful reasoning however
because the decreasing number of votes of $\cpred$ means that
some of the votes from $c_3$ can be changed to $\csec$ as well.
This means that each poisoned sample can reduce the gap by three rather than two.
The adversary therefore needs an extra $\cert^{\rone}_2$ poisoned samples where
\begin{align*}
  \cert^{\rone}_2 := \ceil{\frac{1}{3}\pos{\gap(\bN, \cpred, \csec) - \cert^{\rone}_1}}
  .
\end{align*}

Overall, we will show that the adversary requires $\cert^{\rone}:= \cert^{\rone}_1 + \cert^{\rone}_2$ poisoned samples.

\kpar{Round 2} 
\kr{bug here. why do we see min?}
It can eliminate $\cpred$ in the second round. To do this, it needs
to choose a class $c \in \mC \backslash \{\cpred\}$ and ensure that
\begin{enumerate}
  \item The class $c$ makes it to Round 2.
    Letting $c_2$ denote the second class in Round 1, this requires
    $\cert^{\rtwo, c}_{1} := \ceil{\frac{\gap(\bN^{\rone}, c_2, c)}{2}}$ samples.
  \item In Round 2, $c$ can beat $\cpred$.
    Note that we are effectively assuming that
    $\cpred$ also makes it to Round 2 as $\cpred$ as we have already
    considered the case where $\cpred$ is eliminated in Round 1.
    Define $\bN^{\rtwo, c} := (N^{\rtwo, c}_{\cpred}, N^{\rtwo, c}_{c})$ where
    \begin{align*}
      N^{\rtwo, c}_{\cpred} := \sum_{i=1}^{k} \ind{f_i^{\logit}(x, \cpred) > f_i^{\logit}(x, c)}
      ,
    \end{align*}
    and $N^{\rtwo, c}_{c} := k - N^{\rtwo, c}_{\cpred}$. 
    As before, the adversary requires
    $\cert^{\rtwo, c}$ poisoned samples where
    \begin{align*}
      \cert^{\rtwo, c}_{2} := \ceil{\frac{1}{2}\pos{\gap(\bN^{\rtwo, c}, \cpred, c}}
      .
    \end{align*}
\end{enumerate}
Taking a maximum between the two bounds,
we conclude that the adversary requires
$\cert^{\rtwo}$ poisons where
\begin{align*}
  \cert^{\rtwo} := \min_{c\ne \cpred}\left(\max\left\{\cert^{\rtwo, c}_1, \cert^{\rtwo, c}_2)\right\}\right)
  .
\end{align*}

\kpar{Certificate} Putting everything together, we obtain the following theorem.
\begin{theorem}\label{thm:certificate}
  Given a training set $D$ and an input $x$, 
  define $c, c'$ as in Algorithm \ref{alg:ROE},
  or any training set $D'$, if
  \begin{align*}
    \dsym(D, D') < \min
    \left\{
      \cert^{\rone},
      \cert^{\rtwo}
    \right\}
  .
  \end{align*}
  then Algorithm~\ref{alg:ROE} would still predict $c$ when trained on the dataset $D'$.
\end{theorem}



% \section{Extension to finite aggregation}
% Here, instead of using a single hash function $h: \mathcal{D} \to [k]$, we use
% a set of hash functions $\{h_t\}_{t=1}^{d}$, each mapping $\mathcal{D}$ to $[kd]$. 
% We create $kd$ datasets $D_{1}, \dots D_{kd}$ where $D_i$ contains
% all samples $x$ such that $h_t(x) = i$ for \emph{some $t$}, i.e.,
% \begin{math}
%   D_{i} = \{x | \exists t: h_t(x) = i\}.
% \end{math}
% \footnote{
%   Our explanation here is slightly different from that of~\cite{wang2022improved},
%   where FA is introduced using a \emph{slitting} hash functions $h_{\text{split}}: \mathcal{D} \to [kd]$ and
%   a \emph{spreading} hash function $h_{\text{spread}}: [kd] \to [kd]^d$.
%   Each $D_i$ contains all $x$ such that $i \in h_{\text{spread}}(h_{\text{split}}(x))$.
%   By viewing $h_{\text{spread}}$ as $d$ seperate functions $h_{\text{spread}, i} : [kd] \to [kd]$,
%   we can see that the definitions are equivalent with $h_{i} := h_{\text{split}} \circ h_{\text{spread}, i}$.
% }



Formally, for each bucket $b\in [kd]$, define its \emph{poisoning power with respect to classes $\tilde{c}, c$} as
\begin{align*}
  \pw_{\tilde{c}, c, b} :=
  \sum_{i \in \hspread(b)} 2\ind{f_i(x) = \tilde{c}} + \ind{f_i(x) \ne c}
  .
\end{align*}
The poisoning power measures how much the
adversary can reduce the $\gap(\bNfirst, \tilde{c}, c)$ between $\tilde{c}$ and $c$
by poisoning a sample in bucket $i$ where $\bNfirst$ is the vector of first-round votes of $kd$ models.
Given a budget of $B$ samples to poison,
the reduction in the gap caused by the adversary is no more than
the sum of the top $B$ coordinates in $\pw_{\tilde{c}, c, b}$. 
Note that the upper bound is not necessarily tight since we may be double
counting some partitions \kr{should be models?} $i\in [kd]$. Since we are obtaining a certificate, however, this is not an issue.
By finding the smallest value of $B$ to make the gap non-positive, we obtain a certificate for our prediction.
Formal pseudocode is provided in Algorithm \ref{alg:fa-cert}.

\newcommand{\CertFA}{\textsc{CertFA}}
\newcommand{\mycount}{\textnormal{count}}
\begin{algorithm}
  \caption{FA Certificate algorithm \SF{focus on FA+ROE certificate}}
  \label{alg:fa-cert}
  \begin{algorithmic}[1]
    \Require{Array $\pw$ of size $kd$, an integer $\gap \in \{0\} \cup \mathbb{N}$.}
    \Ensure{Minimum number of poisoned samples needed to make the gap non-positive.}
    \Function{\CertFA}{$\pw, \gap$}
    \State Sort array \pw\ in decreasing order
    \State $\mycount \gets 0$
    \While {\gap $> 0$}
      \State \gap $\gets$ \gap $- \pw_{\mycount}$
      \State $\mycount \gets \mycount + 1$
    \EndWhile
    \State \Return $\mycount$
    \EndFunction
  \end{algorithmic}
\end{algorithm}

\subsection{Finite aggregation + Run-off election}
\label{sec:roe_fa_cert}
As before, we calculate the certificate of our algorithm by considering
the number of poisons required to eliminate $\cpred$ in each of the two rounds.

\kpar{Round 1}
For any fixed classes $c, c'\in \mC \backslash \{\cpred\}$, we bound the number of poisons the adversary requires
in order to ensure that $c, c'$ make beat $\cpred$ in Round 1.
\kb{Add explanation about duality. We need to ensure two constraints.
However, the gap can only look at one thing. We therefore consider the dual definition of the constraints.
}
In order for this to happen, the adversary needs to ensure that
both $\gap(\bNfirst, \cpred, c)$ and $\gap(\bNfirst, \cpred, c')$ are non-positive.
Using the same reasoning as in Finite aggregation, this means
that the adversary needs at least $\max\{\cert^{\rone}_c, \cert^{\rone}_{c'}\}$
samples where
\begin{align*}
  \cert^{\rone}_{c} := \textsc{CertFA}((\pw_{\cpred, c, b})_{b\in [kd]}, \gap(\bNfirst, \cpred, c))
  .
\end{align*}
We can further improve this bound by observing that since 
$\gap(\bNfirst, \cpred, c)$ and $\gap(\bNfirst, \cpred, c')$ both need to be non-positive,
so does their sum $\gap_{c+c'} := \gap(\bNfirst, \cpred, c) + \gap(\bNfirst, \cpred, c')$.
We can similarly bound the poisoning power of the adversary by defining
\begin{align*}
  \pw^{+}_{c, c', b} := 
  \sum_{i\in \hspread(b)} 3\ind{f_i(x) = \cpred} + \ind{f_i(x) \notin (c, c')}
  .
\end{align*}
Defining $\pw^{+}_{c, c'} := (\pw^{+}_{c, c', b})_{b\in [kd]}$,
the adversary requires $\cert^{\rone, +}_{c, c'}$ samples where
\begin{align*}
  \cert^{\rone, +}_{c, c'} := \textsc{CertFA}(\pw_{c, c'}^{+}, \gap_{c+c'}).
\end{align*}
Taking a minimum across all choices of $c, c'$, we obtain the bound
\begin{align*}
  \cert^{\rone} := 
  \min_{c, c' \ne \cpred}\left(
    \max\{\cert_{c, c'}^{\rone, +}, \cert_{c}^{\rone}, \cert_{c'}^{\rone}\}
  \right)
  .
\end{align*}

\kpar{Round 2}
Similar to Section \ref{sec:roe_dpa}, fix a class $c$ and consider
the minimum number of samples the adversary needs to poison
in order to ensure the following. 
\begin{enumerate}
  \item The class $c$ makes it to Round 2.
    This means that
    $c$ needs to beat at least one of
    $\cpred$ and $\csec$. 
    For each, $\tilde{c}\in \{\cpred, \csec\}$,
    we can bound the number of poisons the adversary needs
    to ensure $c$ beats $\tilde{c}$ as
    at least $\cert^{\rtwo}_{c, \tilde{c}}$ poisons where
    \begin{align*}
      \cert^{\rtwo}_{c, \tilde{c}} := \textsc{CertFA}((\pw_{\tilde{c}, c, b})_{b\in [kd]}, \gap(\bNfirst, \tilde{c}, c))
      .
    \end{align*}
    \kb{todo : get rid of min given the discussion with Keivan.}
    Therefore, the adversary requires at least
    $\cert^{\rtwo, c}_{1} := \min\{\cert^{\rtwo}_{c, \cpred}, \cert^{\rtwo}_{c, \csec}\}$ samples to poison.
  \item The class $c$ needs to beat $\cpred$ in Round 2.
    This is similar to a binary version of the original finite aggregation.
    We show that the adversary requires at least
    $\cert^{\rtwo, c}_{2}$ samples where
    $\cert^{\rtwo, c}$ is calculated in the appendix.
    and we defer the details to the appendix.
\end{enumerate}
Taking a maximum between the two rounds, we obtain
the bound $\cert^{\rtwo} := \min_{c \neq \cpred}\left(\max\{\cert^{\rone, c}, \cert^{\rtwo, c}\}\right)$.

\kpar{Certificate} Putting everything together, we obtain the 
same result as DPA, i.e., Theorem \ref{thm:certificate},
with the new values of
$\cert^{\rone}$ and $\cert^{\rtwo}$.

\subsection{Run-off election}



In order to formalize this idea, we introduce the notion of the \emph{gap} between two classes.
Let $\bN := \{\none_c\}_{c\in \mC}$ denote the vector of predictions.
we define the \emph{gap} between $c$ and $c'$ as
\begin{align*}
  \gap(\bN, c, c') := \none_c - \none_{c'} + \ind{c' > c}
  .
\end{align*}
Let $\cpred := DPA(D, x)$ denote the predicted class.
In order to change the model's prediction, the adversary needs to
make the $\gap(\bN, \cpred, c)$ non-positive, for some class $c$. 
Each poisoned sample can only reduce this gap by at most two
since it will decrease $\none_{\cpred}$ by at most one and
increase $\none_{c'}$ by at most one.
As shown in \cite{levine2020deep}, this leads
to a valid certificate as stated by the following theorem.


==> old-notes/old-notes.tex <==
% !TEX root = ../main.tex
\section{Notes}
\cite{carlini2019evaluating}:
More concerning than the fact that progress is slow is the fact that most proposed defenses are quickly 
shown to have performed incorrect or incomplete evaluations.

\begin{enumerate}
  \item DNN + reliability. Strong benchmark. Despite this, widespread use held back by adversarial vulnerabilities.
  \item Broadly speaking, there are two kinds of attacks (explain).
    In this paper, we focus on defenses
    against training time attacks and specifically, data poisoning attacks.
    Define data poisoning (mention accuracy and targeted misclassification?).
  \item Important to be reliable as data hungry and crawling web. Recent work however has been an arm race.
    Attacks and defenses.
  \item Given the importance of building robust models that will not break,
    recent work have proposed considering provable defenses, both for test-time and training-time attacks.
    For data poisoning Levine and Feizi proposed the DPA method.
    Subsequently, Wang et el. obtained improved results by considering more
    general partitioning techniques, though this comes at the extra computational cost.
  \item In this work, we propose a simple method that significantly outperforms existing baselines
    \emph{without extra computation cost}.
    The key idea behind our method is to \emph{utilize logits-layer information of the models for prediction.}
    On the Cifar-10 dataset, we outperform
    the FA upon the results of Wang et al. with
    \textbf{32 times less computational cost.}
    We further extend our methodology to more complicated partitioning schems simliar to
    Wang et al., and obtain additional improvements in these settings.
\end{enumerate}

Questions:
Intro:
\begin{enumerate}
  \item Who should we cite in the intro?
  \item What numbers to report and what should we say?
\end{enumerate}
Related work:
\begin{enumerate}
  \item Should we discuss anything else such as attacks and defense?
  \item Should we discuss all of th (Diakonikolas stuff?
\end{enumerate}

\section{Old Introduction}

In recent years, Deep Neural Networks (DNNs) have achieved great success in many research areas,
especially computer vision \cite{he2016deep} and natural language processing \cite{chen2015convolutional}. 
This significant improvement in the performance of DNNs is mainly
due to the accessibility of more powerful computational resources
and the availability of bigger and better datasets to train these networks. 
However, having access to many data sources increases
the risk of using unreliable or even poisoned data that can
adversly affect the reliability of networks,
which raises questions about the vulnerability of DNNs.


In this work, we consider data poisoning in classification problem,
which is a process that an adversary
purposely adds or removes some data to
manipulate the  model's behavior at test time.
The goal of data poisoning is mostly to corrupt a classifier's 
performance on one specific test instance or a class of data points.
This is targeted attack, which has been widely investigated in the recent data poisoning literature. 
\cite{chen2017targeted, gao2021learning, shafahi2018poison} are all examples of targeted data 
poisoning.

There are two categories of data poisoning attacks: Some attacks are performed on test data 
called evasion attacks. These attacks rely on generating adversarial examples capable of 
manipulating a classifier with minor modifications to the test data. Other poisoning 
attacks are performed on train data. They inject some adversarially perturbed 
samples into the train set to alter the DNN's classification predictions. 
As mentioned before, due to the availability of many data sources and the 
unsupervised manner of gathering data to train models, the latter data 
poisoning method has been more investigated by researchers.

 
Many defense mechanisms have been developed against data poisoning attacks,
such as Data Augmentation and Data Sanitization-based methods.
The former
uses models which are trained on bigger training sets
achieved by different techniques of data augmentation \cite{ni2021data, gong2020maxup},
which enables models to be more robust against data poisoning attacks \cite{borgnia2021strong}, 
and the latter
uses anomaly detectors to filter out suspicious training points from clean data
clean data 
\cite{paudice2018label, hodge2004survey, cretu2008casting}.
% \cite{ni2021data, gong2020maxup}

An important questions that is raised here is that:
are there defenses that are robust to a large class of data poisoning attacks?
Typically, one could take a clean dataset and utilize a defense technique, and then
test the trained model on a limited number of poisoning strategies on that dataset.
However, since there can be unlimited ways to come up with poisoning attacks, 
it is impossible to conclude from empirical success alone
that a defense that works well on a limited number of known attacks
will still perform well agains new attacks,
which emphasizes on the importance developing provably robust defenses
such that no matter how poisoning attacks are being done, 
we can still rely on our models.

In provably robust methods,
we want the prediction of the model
remains unchanged within a specific attack size. 
The previous methods based on data augmentation and sanitization
do not perform well compared to methods based on \textbf{Data Aggregation}, 
which offers pointwise certified robustness against poisoning attacks via
majority voting for each data sample. One example of such a defense 
mechanism is Deep Partition Aggregation \cite{levine2020deep}. 
They propose an ensemble-based certified classifier that divides 
the training data into disjoint subsets and feeds these subsets 
into its independent deterministic submodels. Another example is 
Finite Aggregation \cite{wang2022improved} which outperforms DPA
by using a more complex structure to feed training dataset to submodels.

We proposed an aggregation-based data poisoning defense called 
\textbf{Run-off election} that frequently outperforms the proposed 
Finite Aggregation method of \cite{wang2022improved}, while 
\textbf{using 32 times less computational resources}. Our 
accuracy gain with the same setting as DPA and Finite 
Aggregation on MNIST is \textbf{$\sim$ +4.73\%} 
and \textbf{$\sim$ +6.06\%} comparing to DPA and 
Finite Aggregation respectively.

\section{Old Related work}
Our work is inspired mainly by the Deep Partition Aggregation (DPA) framework
\cite{levine2020deep} and the Finite Aggregation method \cite{wang2022improved}. The former
is an aggregation-based authentication defense method that partitions the training data
into disjoint subgroups and feeds each subgroup individually into a classification model.
It uses the majority vote of all models to predict the final classification of a given
input. The latter considers point-wise certified robustness and extends DPA by partitioning
the training dataset into smaller disjoint subsets and then combining these subsets to
create larger subsets that share some training data. It then uses these subsets for
training classifiers. Their results show some improvement over DPA.

In addition, \cite{steinhardt2017certified} proposed a distributional defense against
poisoning attacks, a well-known framework in defenses against poisoning data.
\cite{steinhardt2017certified} can guarantee a certain level of accuracy on test data only
if it is driven from the same distribution as the clean training data. Some previous works,
such as \cite{diakonikolas2016new, lai2016reducing} offer distributional guarantees for
unsupervised learning methods under poisoning attacks. Their other work
\cite{diakonikolas2019sever} approximates the clean-trained model under some assumptions
over the distribution of the clean train set.

In the context of randomized smoothing, some defense mechanisms, such as
\cite{weber2020rab} applies \cite{cohen2019certified}'s smoothing L2 evasion defense to the
poisoning domain. However, this defense method has three main limitations. Firstly, it only
certifies clean-label attacks, which lowers their generality to other attacks, such as
backdoor attacks with modified labels \cite{chen2017targeted}. Secondly, since it uses L2
evasion, it cannot certify poisoning attacks further than the bound of the L2 norm. Thirdly
\cite{weber2020rab} proposed a randomized certificate instead of a deterministic one when
using deep classifiers, and the error approaches zero only when the number of classifiers
goes to infinity. Other limitations of smoothing-based methods are further discussed in
\cite{yang2020randomized, kumar2020curse, blum2020random}.

==> old-notes/trash.tex <==
% !TEX root = ../main.tex
Intuitively, 
letting $c$ denote the final output,
and let $c'$ denote the other class in Round 1, i.e.,
$\{c, c'\} = \{c_1, c_2\}$,
the adversary can change the final prediction in three ways.
\kr{Why? I know it is obvious that
these three cases give the adversary
minimum number of poisons he needs,
but there are other ways that he can change the prediction.
We should say that those other cases are not optimal.
}
\begin{enumerate}
  \item It can change the output to $c'$
    by ensuring that $c'$ beats $c$ in Round 2.
    This is basically a DPA poisoning problem
    with $k$ models and two classes $c, c'$. 
    Using a simliar argument as in Theorem \ref{thm:dpa}
    we show that
    the minimum number of poisons 
    for changing the prediction equals
    % the adversary needs more than $\cert_1$ poisoned samples,
    % which equals
    \begin{align*}
      \cert_1 \gets \floor{\frac{1}{2}\left(\nrun_c - \nrun_{c'} - \ind{c' < c}\right) } + 1.
    \end{align*}
  \item It can change the output of the first round
    such that $c$ is no longer in Round 2.
    As we will show,
    this means that the adversary needs to choose a class $\tilde{c}$
    and ensure that $N_{c} \le \min\{N_{c'}, N_{\tilde{c}}\}$.
    The minimum number of poisons can therefore be calculated using a simple water-filling argument.
    To achieve this, the adversary should keep changing the $c$ predictions to $c'$
    until $c'$ beats $c$, and should then repeat the same
    procedure with $\tilde{c}$.
    Formally, we set $\cert_2 := \cert_{2}' + \max\{0, \wtilde{\cert_{2}}\}$ where
    \begin{align*}
      &\cert_2' := \floor{\frac{1}{2}\left(N_c - N_{c'} - \ind{c' < c}\right) } + 1, \\
      &\wtilde{\cert_{2}} := \floor{\frac{1}{2}\left(N_c -\cert_2' - N_{\tilde{c}} - \ind{\tilde{c} < c}\right)} + 1
      .
    \end{align*}
  \item It can change the output to some $\tilde{c}\notin \{c, c'\}$
    by ensuring that $(c, \tilde{c})$ are outputed in Round 1
    \emph{and} $\tilde{c}$ beats $c$ in Round 2.
    The number of poisons for the each of these steps
    can be calculated using a simliar argument as DPA.
    Formally, 
    defining $\nruntilde_{c} := \sum_{i=1}^{k} \ind{f_i^{\logit}(c) > f_i^{\logit}(\tilde{c})}$ and $\nruntilde_{\tilde{c}} := k - \nruntilde_{c}$,
    we set $\cert_3 := \max\{\cert_3', \cert_3^{\runoff}\}$,
    where
    \begin{align*}
      &\cert_3' := \floor{\frac{1}{2}\left(N_{c'} - N_{\tilde{c}} - \ind{\tilde{c} < c'}\right) } + 1, \\
      &\cert_3^{\runoff} := \floor{\frac{1}{2}\left(\nruntilde_{c} - \nruntilde_{\tilde{c}} - \ind{\wtilde{c} < c'}\right) } + 1.
    \end{align*}
\end{enumerate}
For each of these cases, we calculate a lower bound
on the number of poisons needed for the change mechanism.
Taking a minimum over the three numbers provides a lower bound
on the number of the robustness certificate.
Formally, we obtain the following theorem.

\begin{theorem}
  Given a training set $D$ and an input $x$, 
  define $c, c'$ as in Algorithm \ref{alg:election},
  jor any training set $D'$, if
  \begin{align*}
    \dsym(D, D') < \min\{\cert_1, \cert_2, \cert_3\}
    ,
  \end{align*}
  then Algorithm \ref{alg:election} would still predict $c$ when trained on the dataset $D'$.
\end{theorem}


\subsection{old}
Since any poisoned training sample can affect at most a single base model,
the overall prediction would \emph{provably} remain the same
as long as the number of poisoned samples is not large enough 
to overcome the margin between the top class and the runner up class, i.e., the class with the second-highest
number of votes.

\kr{After giving a more general intuition of our work,
  we can compare it with DPA and say something like below.}

To address this issue, we propose a novel aggregation method by using \emph{the logits-layer information} of the models.
We view the aggregation phase as an election,
where each base model corresponds to a voter
and has an underlying score indicating how much it favors each class.
These scores can be obtained by, e.g., considering
the logits-layer of the base classifers.
Under the new election view,
we can see the approach taken by prior work corresponds
to a ``first-past-post'' election, where it is known that
voters not voting for the top choices are effectively ignored.
This effectively limits the number of base models utilized in the prediction process.
We address this issue by considering a \emph{two-round} election process.
In the first round, the models first vote for their preferred class
and we obtain the top-two classes in terms of number of votes.
We then hold a \emph{second round} where
each of the base models vote for one of these two classes by
choosing the class with the higher underlying score.
An illuatrative example of our approach is shown in Figure \ref{fig:main_fig}.

\kr{I think we previously had something like multi-label classification is harder
  than binary classiciation which was a really nice intuition. We should have kept that.
  Here, we also write something regarding that this run-off election method is harder.
  to analyze as we need to consider both two rounds,
  it is not as simple as DPA where we only considere 2nd class}

By using the full logit-layer information for each model,
we are effectively increasing the number of base classifiers
which play a role in the final output of the model, 
and therefore increasing the effective \emph{margin} of our prediction method.
This \emph{dilutes} the adversary's power
as it needs to use more poisoned samples
to change our prediction.

\kr{We need to be consistent for adversary budget notation $B$, or $b$?}

\kb{Write about the wattr-filling method. Write about the duality argument.}


==> tables/intro.tex <==
% !TEX root = ../main.tex
\begin{table}[H]
    \caption{
        Training cost, and provable accuracy of different methods when
        the adversary is allowed to manipulate at most $400$ samples of MNIST training dataset.
    }
    \vskip 0.15in
    \label{table:intro}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|c}
        training cost & method & accuracy\\ 
        \hline
        \multirow{2}{*}{1}  &   \footnotesize{DPA}        &   61.78\% \\\cline{2-3}
                            &   \footnotesize{ROE + DPA}  &   \textbf{65.42\%}{\color{blue}(+3.64\%)} \\\cline{1-3}
        \multirow{2}{*}{32} &   \footnotesize{FA}         &   64.34\%{\color{blue}(+2.56\%)} \\\cline{2-3}
                            &   \footnotesize{ROE + FA}   &   \textbf{66.72\%}{\color{blue}(+4.94\%)} \\%\cline{1-3}       
    \end{tabular}}
\end{table}

==> tables/result_stats.tex <==
% !TEX root = ../main.tex
\begin{table*}[tb]
\caption{
    Certified fraction of Run-off election, and Finite-Aggregation with different values of $d$ with respect to different attack sizes $B$.
    The improvements compared to the DPA baseline are highlighted in blue if they are positive and red otherwise.
}
\vskip 0.15in
\label{table:result_stats}
% \resizebox{16cm}{!}{
\resizebox{1\linewidth}{!}{ % revise {h_size}{v_size} to adjust the overall size of the table
  \begin{tabular}{|c||c||c|c||c|c|c|c|c|}
   \hline
      model & $k$ & method & $d$ & \multicolumn{5}{|c|}{certified fraction}\\ 
      \hline\hline
      \multirow{6}{*}{MNIST}       & \multirow{6}{*}{1200}    & \multicolumn{2}{c||}{}                      & $B\leq 100$ & $B\leq 200$ & $B\leq 300$ & $B\leq 400$ & $B\leq 500$\\\cline{3-9}
                                   &                          & \multirow{3}{*}{FA} & 1 (DPA)               & 92.11\% & 86.45\% & 77.12\% & 61.78\% & 32.42\%\\\cline{4-9}
                                   &                          &                     & 8                     & 92.45\%{\color{blue}(+0.34\%)} & 86.97\%{\color{blue}(+0.52\%)} & 77.31\%{\color{blue}(+0.19\%)} & 61.81\%{\color{blue}(+0.03\%)} & 32.30\%{\color{red}(-0.12\%)}\\\cline{4-9}
                                   &                          &                     & 16                    & 92.75\%{\color{blue}(+0.64\%)} & 87.89\%{\color{blue}(+1.44\%)} & 78.91\%{\color{blue}(+1.79\%)} & 62.42\%{\color{blue}(+0.64\%)} & 31.97\%{\color{red}(-0.45\%)}\\\cline{4-9}
                                   &                          &                     & 32                    & 92.97\%{\color{blue}(+0.86\%)} & 88.49\%{\color{blue}(+2.04\%)} & 80.17\%{\color{blue}(+3.05\%)} & 64.34\%{\color{blue}(+2.56\%)} & 31.09\%{\color{red}(-1.33\%)}\\\cline{3-9}
                                   &                          & \multicolumn{2}{c||}{Run-off election}      & 92.40\%{\color{blue}(+0.29\%)} & 87.46\%{\color{blue}(+1.01\%)} & 79.44\%{\color{blue}(+2.32\%)} & 65.42\%{\color{blue}(+\textbf{3.64}\%)} & 37.15\%{\color{blue}(+\textbf{4.73}\%)}\\\cline{3-9}
      \hline\hline
      \multirow{12}{*}{CIFAR-10}   & \multirow{6}{*}{50}      & \multicolumn{2}{c||}{}                      & $B\leq 5$ & $B\leq 10$ & $B\leq 15$ & $B\leq 18$ & $B\leq 20$\\\cline{3-9}
                                   &                          & \multirow{4}{*}{FA} & 1 (DPA)               & 58.07\% & 46.44\% & 33.46\% & 24.87\% & 19.36\% \\\cline{4-9}
                                   &                          &                     & 8                     & 59.80\%{\color{blue}(+1.73\%)} & 47.40\%{\color{blue}(+0.96\%)} & 33.76\%{\color{blue}(+0.30\%)} & 25.45\%{\color{blue}(+0.58\%)} & 19.72\%     {\color{blue}(+0.36\%)}\\\cline{4-9}
                                   &                          &                     & 16                    & 60.55\%{\color{blue}(+2.48\%)} & 48.85\%{\color{blue}(+2.41\%)} & 34.61\%{\color{blue}(+1.15\%)} & 25.46\%{\color{blue}(+0.59\%)} & 19.90\%{\color{blue}(+0.54\%)}\\\cline{4-9}
                                   &                          &                     & 32                    & 61.31\%{\color{blue}(+3.24\%)} & 50.31\%{\color{blue}(+3.87\%)} & 36.03\%{\color{blue}(+2.57\%)} & 26.55\%{\color{blue}(+1.68\%)} & 19.93\%{\color{blue}(+0.57\%)}\\\cline{3-9}
                                   &                          & \multicolumn{2}{c||}{Run-off election}      & 59.85\%{\color{blue}(+1.78\%)} & 49.15\%{\color{blue}(+2.71\%)} & 36.08\%{\color{blue}(+\textbf{2.62}\%)} & 27.52\%{\color{blue}(+\textbf{2.65}\%)} & 21.30\%{\color{blue}(+\textbf{1.94}\%)}\\\cline{2-9}
                                   & \multirow{6}{*}{250}     & \multicolumn{2}{c||}{}                      & $B\leq 10$ & $B\leq 20$ & $B\leq 40$ & $B\leq 50$ & $B\leq 60$\\\cline{3-9}
                                   &                          & \multirow{4}{*}{FA} & 1 (DPA)               & 44.31\% & 34.01\% & 18.99\% & 13.55\% & 9.25\%\\\cline{4-9}
                                   &                          &                     & 5                     & 44.83\%{\color{blue}(+0.52\%)} & 34.92\%{\color{blue}(+0.91\%)} & 19.42\%{\color{blue}(+0.43\%)} & 13.92\%{\color{blue}(+0.37\%)} & 9.61\%{\color{blue}(+0.36\%)}\\\cline{4-9}
                                   &                          &                     & 8                     & 45.38\%{\color{blue}(+1.07\%)} & 36.05\%{\color{blue}(+2.04\%)} & 20.08\%{\color{blue}(+1.09\%)} & 14.39\%{\color{blue}(+0.84\%)} & 9.70\%{\color{blue}(+0.45\%)}\\\cline{4-9}
                                   &                          &                     & 16                    & 46.52\%{\color{blue}(+2.21\%)} & 37.56\%{\color{blue}(+3.55\%)} & 21.99\%{\color{blue}(+3.0\%)} & 15.79\%{\color{blue}(+2.24\%)} & 11.09\%{\color{blue}(+1.84\%)}\\\cline{3-9}
                                   &                          & \multicolumn{2}{c||}{Run-off election}      & 46.23\%{\color{blue}(+1.92\%)} & 38.13\%{\color{blue}(+\textbf{4.12}\%)} & 23.33\%{\color{blue}(+\textbf{4.34}\%)} & 17.68\%{\color{blue}(+\textbf{4.13}\%)} & 12.49\%{\color{blue}(+\textbf{3.24}\%)}\\\cline{2-9}
      \hline\hline
      \multirow{10}{*}{GTSRB}      & \multirow{6}{*}{50}      & \multicolumn{2}{c||}{}                      & $B\leq 5$ & $B\leq 10$ & $B\leq 15$ & $B\leq 20$ & $B\leq 22$\\\cline{3-9}
                                   &                          & \multirow{3}{*}{FA} & 1 (DPA)               & 82.32\% & 74.15\% & 64.14\% & 49.12\% & 37.73\%\\\cline{4-9}
                                   &                          &                     & 16                    & 82.71\%{\color{blue}(+0.39\%)} & 74.66\%{\color{blue}(+0.51\%)} & 63.77\%{\color{red}(--0.37\%)} & 47.52\%{\color{red}(--1.6\%)} & 35.54\%{\color{red}(--2.19\%)}\\\cline{4-9}
                                   &                          &                     & 32                    & 83.52\%{\color{blue}(+1.2\%)} & 76.26\%{\color{blue}(+2.11\%)} & 66.32\%{\color{blue}(+2.18\%)} & 49.68\%{\color{blue}(+0.55\%)} & 38.31\%{\color{blue}(+0.59\%)}\\\cline{3-9}
                                   &                          & \multicolumn{2}{c||}{Run-off election}      & 82.66\%{\color{blue}(+0.34\%)} & 74.94\%{\color{blue}(+0.79\%)} & 66.03\%{\color{blue}(+1.89\%)} & 51.34\%{\color{blue}(+\textbf{2.22}\%)} & 39.18\%{\color{blue}(+\textbf{1.45}\%)}\\\cline{2-9}
                                   & \multirow{6}{*}{100}     & \multicolumn{2}{c||}{}                      & $B\leq 10$ & $B\leq 20$ & $B\leq 28$ & $B\leq 35$ & $B\leq 42$\\\cline{3-9}
                                   &                          & \multirow{4}{*}{FA} & 1 (DPA)               & 46.16\% & 38.24\% & 30.19\% & 22.84\% & 20.34\%\\\cline{4-9}
                                   &                          &                     & 16                    & 48.19\%{\color{blue}(+2.03\%)} & 41.62\%{\color{blue}(+3.37\%)} & 33.95\%{\color{blue}(+3.76\%)} & 25.96\%{\color{blue}(+3.12\%)} & 22.75\%{\color{blue}(+2.41\%)}\\\cline{4-9}
                                   &                          &                     & 32                    & 48.39\%{\color{blue}(+2.23\%)} & 42.01\%{\color{blue}(+3.77\%)} & 34.96\%{\color{blue}(+4.77\%)} & 27.05\%{\color{blue}(+4.2\%)} & 23.82\%{\color{blue}(+3.48\%)}\\\cline{3-9}
                                   &                          & \multicolumn{2}{c||}{Run-off election}      & 46.14\%{\color{red}(--0.02\%)} & 40.10\%{\color{blue}(+1.85\%)} & 33.71\%{\color{blue}(+3.52\%)} & 27.18\%{\color{blue}(\textbf{+4.34}\%)} & 24.76\%{\color{blue}(+\textbf{4.42}\%)}\\\cline{3-9}
      \hline\hline
   
  \end{tabular}
  }
\end{table*}

